GAMIN: An Adversarial Approach to Black-Box Model Inversion

Recent works have demonstrated that machine learning models are vulnerable to model inversion attacks, which lead to the exposure of sensitive information contained in their training dataset. While some model inversion attacks have been developed in the past in the black-box attack setting, in which the adversary does not have direct access to the structure of the model, few of these have been conducted so far against complex models such as deep neural networks. In this paper, we introduce GAMIN (for Generative Adversarial Model INversion), a new black-box model inversion attack framework achieving significant results even against deep models such as convolutional neural networks at a reasonable computing cost. GAMIN is based on the continuous training of a surrogate model for the target model under attack and a generator whose objective is to generate inputs resembling those used to train the target model. The attack was validated against various neural networks used as image classifiers. In particular, when attacking models trained on the MNIST dataset, GAMIN is able to extract recognizable digits for up to 60% of labels produced by the target. Attacks against skin classification models trained on the pilot parliament dataset also demonstrated the capacity to extract recognizable features from the targets.

==> 06-futureWork.tex <==
\section{Future work}
\label{sec:futureWork}

We believe that the GAMIN can still be improved to further improve accuracy or to decrease the high cost of this attack in terms of queries.
The GAMIN could benefit from being tested against targets trained on different types of data, either as inputs (\emph{i.e.}, sequential data for instance) or as outputs (\emph{i.e.}, regressors).
Further development of this architecture could allow for instance a single GAMIN to invert multiple outputs. 
In this case, the cost of the attack would not decrease directly, but a single attack could invert multiple classes, which would dramatically reduce the cost of inverting all classes of the model.
Many developments in adversarial training could also be adapted on the GAMIN to accelerate its convergence, which is another approach for reducing the cost of the model inversion attack.
Finally, a detailed study of countermeasures and their impact of target models depth would be an invaluable addition to the field of model inversion.
Rounding or hiding confidence values, which is one of Fredrikson \coauth{} 's propositions \cite{Fredrikson15}, could be a start, even if when applied to Tramèr \coauth 's attack, it only resulted in an augmentation of the attack cost \cite{Tramer16}. 
%Seb: ci-dessus, je suggère de donner quelques exemples de contre-mesures existantes qui pourrait aussi être appliqués au GAMIN
%Timon: done (mais court)

==> algos/gamin_tikz.tex <==
\begin{figure}[h!]
\begin{tikzpicture}[node distance=1.5cm, every node/.style={fill=white, font=\sffamily}, align=center]
\node (noiseBlock) [] {Noise $z$};
\node (generatorBlock) [redbox, below of=noiseBlock, yshift=0.5cm] {Generator $\generator{}$};
\draw [->] (noiseBlock) -- (generatorBlock);
\node (inputBlock) [below of=generatorBlock, yshift=0.5cm] {Generated inputs $x_\generator{} = \generator{}(z)$};
\draw (generatorBlock) -- (inputBlock);
\node (voidInputBlock) [below of=inputBlock, yshift=0.75cm] {};
\node (targetBlock) [blackbox,below of=voidInputBlock, yshift=0.75cm] {Target model $\targetModel{}$};
\node (voidSepBlock) [right of=targetBlock] {};
\node (shadowBlock) [greybox,right of=voidSepBlock, xshift=-0.15cm] {Surrogate $S$};
\draw (inputBlock) -- (voidInputBlock.center);
\draw [->] (voidInputBlock.center) -- (targetBlock);
\draw [->] (voidInputBlock.center) -| (shadowBlock);
\node (targetOutputBlock) [below of=targetBlock, yshift=0.5cm] {$y=\targetModel{}(x_G)$};
\draw (targetBlock) -- (targetOutputBlock);
\node (voidYSepBlock) [below of= voidSepBlock, yshift=0.5cm] {};
\draw (targetOutputBlock) -- (voidYSepBlock.center);
\node (shadowOutputBlock) [below of=shadowBlock, yshift=0.5cm] {$\hat{y}=S(x_G)$};
\draw (shadowBlock) -- (shadowOutputBlock);
\draw (voidYSepBlock.center) -- (shadowOutputBlock);
\node (voidY2SepBlock) [right of=shadowOutputBlock, xshift=-0.25cm] {};
\node (y0Block) [right of=voidY2SepBlock, xshift=-0.5cm] {Target $\targetOutput{}$};
\draw (voidY2SepBlock.center) -- (shadowOutputBlock);
\draw (voidY2SepBlock.center) -- (y0Block);
\draw [->] (voidYSepBlock.center) |- (shadowBlock);
\draw [->] (voidY2SepBlock.center) |- (generatorBlock);
\end{tikzpicture}
\centering
\caption{GAMIN attack process} 
\label{fig:gamin:schema}
\end{figure}


==> algos/gan.tex <==
\begin{algorithm}[h!]
\caption{GAN training} % commenter cette ligne pour faire disparaître l'erreur mystère
\label{algo:gan-train} % commenter cette ligne pour faire disparaître l'erreur mystère
\begin{algorithmic}%[1]
\Require ($G$, $\theta_G$) generator model, ( $D$, $\theta_D$) discriminator model, $T$ training set 
\For {$n$ epochs} 
\Statex   \Comment {Generate artificial inputs from noise}
%\State \textit{\# Generate artificial inputs from noise}
\State $z \sim \mathcal{N}(0,1)$
\State $X_G \gets G_{\theta_G}(z)$
\Statex   \Comment {Mix with true inputs from training set}
%\State \textit{\# Mix with true inputs from training set}
\State $X_T \sim T$
\Statex   \Comment {Train discriminator}
%\State \textit{\# Train discriminator}
\State $\theta_D \gets train(X_G, False)$
\State $\theta_D \gets train(X_T, True)$
\Statex   \Comment {Train generator based on discriminator error propagation}
%\State \textit{\# Train generator based on discriminator error propagation}
\State $\theta_G \gets train(D(G(z)), True)$
\EndFor
\end{algorithmic} 
\end{algorithm}

==> algos/ganB.tex <==
\begin{algorithm}
\caption{GAN training}[h1]
\label{algo:gan-train}
\begin{algorithmic}[1]
\Require ($G$, $\theta_G$) generator model, ( $D$, $\theta_D$) discriminator model, $T$ training set 
\For {$n$ epochs} 
\Statex   \Comment {Generate artificial inputs from noise}
%\State \textit{\# Generate artificial inputs from noise}
\State $z \sim \mathcal{N}(0,1)$
\State $X_G \gets G_{\theta_G}(z)$
\Statex   \Comment {Mix with true inputs from training set}
%\State \textit{\# Mix with true inputs from training set}
\State $X_T \sim T$
\Statex   \Comment {Train discriminator}
%\State \textit{\# Train discriminator}
\State $\theta_D \gets train(X_G, False)$
\State $\theta_D \gets train(X_T, True)$
\Statex   \Comment {Train generator based on discriminator error propagation}
%\State \textit{\# Train generator based on discriminator error propagation}
\State $\theta_G \gets train(D(G(z)), True)$
\EndFor
\end{algorithmic} 
\end{algorithm}

==> algos/survey.tex <==
\resizebox {0.9\columnwidth} {!} {
\begin{tikzpicture}[trim axis left, trim axis right]
\begin{axis}[
    ybar,
    enlarge x limits = 0.06,
    x=1.5cm,
    y=8cm,
    bar width = 0.15cm,
    axis x line*=bottom,
    legend style={%
    	at={(0.5,-0.1)},
      anchor=north,
      legend columns=-1,
      column sep=0.1cm,
      draw=none,
      /tikz/every odd column/.append style={column sep=0cm},
      },
    %ylabel={proportion of correct inference},
    %every axis y label/.style={
    %at={(ticklabel* cs:1.05)},
    %anchor=south,
    %},
    title={proportion of correct inference},
    ymin = 0,
    ymax = 1, 
    symbolic x coords={0, 1, 2, 3, 4, 5, 6, 7, 8, 9},  %TT: c'est là qu'on définit le nb d'ensemble de colonnes
    xtick=data,
    %nodes near coords,
    %nodes near coords align={vertical},
    legend image code/.code={%
                    \draw[#1, draw=black] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
                    }
    ]
\addplot[draw=black, fill=white] coordinates {(0,0.86) (1,0.71) (2,0.86) (3,1) (4,0.43) (5,0.79) (6,0.26) (7,0.64) (8,0.64) (9,0.5)};
\addplot[fill=gray!50] coordinates {(0,0.07) (1,0.0) (2,0.98) (3,1) (4,0.54) (5,0.8) (6,0.54) (7,0.87) (8,0.94) (9,0.04)};
\addplot[fill = gray] coordinates {(0,0.24) (1,0.2) (2,0.94) (3,1) (4,0.44) (5,0.79) (6,0.35) (7,0.82) (8,0.89) (9,0.18)};
\addplot[pattern = north east lines] coordinates {(0,0.29) (1,0.2) (2,0.86) (3,1) (4,0.4) (5,0.4) (6,0.28) (7,0.86) (8,0.71) (9,0.14)};
\addplot[pattern = dots] coordinates {(0,0.53) (1,0.) (2,0.) (3,0.68) (4,0.) (5,0.53) (6,0.) (7,0.05) (8,0.05) (9,0.)};
\legend{Soft, MLP1, MLP2, CNN1, CNN2}
\end{axis}
\end{tikzpicture}
}

==> algos/survey_majority.tex <==
\begin{figure}[h!]
\centering
\resizebox {0.85\columnwidth} {!} {
\begin{tikzpicture}[trim axis right]
\begin{axis}[
    ybar,
    %enlargelimits=0.15,
    enlarge x limits = 0.45,
    axis x line*=bottom,
    y=6cm,
    legend style={%
    	at={(0.5,-0.15)},
      anchor=north,
      legend columns=-1,
      column sep=0.1cm,
      draw=none,
      /tikz/every odd column/.append style={column sep=0cm},
      },
    title={Proportion of correct inferences},
    %ylabel={proportion of correct inference},
    ymin = 0,
    ymax = 1, 
    symbolic x coords={average,majority},  %TT: c'est là qu'on définit le nb d'ensemble de colonnes
    xtick=data,
    %nodes near coords,
    %nodes near coords align={vertical},
    legend image code/.code={%
                    \draw[#1, draw=black] (0cm,-0.1cm) rectangle (0.2cm,0.1cm);
                    }
    ]
\addplot[draw=black, fill=white] coordinates {(average,0.67) (majority,0.8)};
\addplot[fill=gray!50] coordinates {(average,0.58) (majority,0.7)};
\addplot[fill = gray] coordinates {(average,0.49) (majority,0.5)};
\addplot[pattern = north east lines] coordinates {(average,0.35) (majority,0.5)};
\addplot[pattern = dots] coordinates {(average,0.18) (majority,0.3)};
\legend{Soft, MLP1, MLP2, CNN1, CNN2}
\end{axis}
\end{tikzpicture}
}
\caption{Results of the survey for MNIST-based models attack. For each target model, the average (over all the target digits) of the proportion of correct identification is given as well as the proportion of target digits with at least 50\% of correct identification. }\label{fig:result:mnist:survey1}
\end{figure}

==> tables/dpSurvey.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|}
\hline
\multirow{2}{*}{Target digit} & \multirow{2}{*}{\% correct} \\
 &  \\ \hline
0 & 0.6875 \\ \hline
1 & 0.4375 \\ \hline
2 & 0.7500 \\ \hline
3 & 0.8125 \\ \hline
4 & 0.4375 \\ \hline
5 & 0.9375 \\ \hline
6 & 0.6250 \\ \hline
7 & 0.6875 \\ \hline
8 & 0.3750 \\ \hline
9 & 0.7500 \\ \hline
\end{tabular}
\caption{Result of a survey with 16 participants accessing the results of an inversion attack on a MLP model trained with differential privacy. 
For each of the target digit, the proportion of users who identifies it correctly to the actual class is given.}
\label{tab:dpSurvey}
\end{table}
